JRDB-PanoTrack: An Open-world Panoptic Segmentation and Tracking Robotic Dataset in Crowded Human Environments

Autonomous robot systems have attracted increasing research attention in recent years, where environment understanding is a crucial step for robot navigation, human-robot interaction, and decision. Real-world robot systems usually collect visual data from multiple sensors and are required to recognize numerous objects and their movements in complex human-crowded settings. Traditional benchmarks, with their reliance on single sensors and limited object classes and scenarios, fail to provide the comprehensive environmental understanding robots need for accurate navigation, interaction, and decision-making. As an extension of JRDB dataset, we unveil JRDB-PanoTrack, a novel open-world panoptic segmentation and tracking benchmark, towards more comprehensive environmental perception. JRDB-PanoTrack includes (1) various data involving indoor and outdoor crowded scenes, as well as comprehensive 2D and 3D synchronized data modalities; (2) high-quality 2D spatial panoptic segmentation and temporal tracking annotations, with additional 3D label projections for further spatial understanding; (3) diverse object classes for closed- and open-world recognition benchmarks, with OSPA-based metrics for evaluation. Extensive evaluation of leading methods shows significant challenges posed by our dataset.

==> rebuttal.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}
% \usepackage[rebuttal]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}

% % Import additional packages in the preamble file, before hyperref
% \input{preamble}

% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
% \usepackage[pagebackref,breaklinks,colorlinks,citecolor=cvprblue]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% \newcommand{\Rone}{{{\color{brown} \textbf{R\#NcrU}}}}
% \newcommand{\Rtwo}{{{\color{blue} \textbf{R\#4T3b}}}}
% \newcommand{\Rthree}{{{\color{red} \textbf{R\#RNb3}}}}
% \newcommand{\Rones}{{{\color{brown} \textbf{R\#NcrU }}}}
% \newcommand{\Rtwos}{{{\color{blue} \textbf{R\#4T3b }}}}
% \newcommand{\Rthrees}{{{\color{red} \textbf{R\#RNb3 }}}}

% \newcommand{\ospapt}{$\mathcal{O}^2_{PT}$}
% \newcommand{\ospaptk}{$\mathcal{O}^{2K}_{PT}$}
% \newcommand{\ospaptu}{$\mathcal{O}^{2U}_{PT}$}
% \newcommand{\ospapts}{$\mathcal{O}^{2S}_{PT}$}
% \newcommand{\ospaptt}{$\mathcal{O}^{2T}_{PT}$}
% \newcommand{\ospaptbold}{$\bm{\mathcal{O}}^{\textbf{2}}_{\textbf{PT}}$}
% \newcommand{\ospaptboldl}{$\bm{\mathcal{O}}^{\textbf{2}}_{\textbf{\textit{Loc}}}$}
% \newcommand{\ospaptboldc}{$\bm{\mathcal{O}}^{\textbf{2}}_{\textbf{\textit{Card}}}$}
% \newcommand{\ospaptboldk}{$\bm{\mathcal{O}}^{\textbf{2K}}_{\textbf{PT}}$}
% \newcommand{\ospaptboldu}{$\bm{\mathcal{O}}^{\textbf{2U}}_{\textbf{PT}}$}
% \newcommand{\ospaptboldt}{$\bm{\mathcal{O}}^{\textbf{2T}}_{\textbf{PT}}$}
% \newcommand{\ospaptbolds}{$\bm{\mathcal{O}}^{\textbf{2S}}_{\textbf{PT}}$}

% % If you wish to avoid re-using figure, table, and equation numbers from
% % the main paper, please uncomment the following and change the numbers
% % appropriately.
% %\setcounter{figure}{2}
% %\setcounter{table}{1}
% %\setcounter{equation}{2}

% % If you wish to avoid re-using reference numbers from the main paper,
% % please uncomment the following and change the counter for `enumiv' to
% % the number of references you have in the main paper (here, 6).
% %\let\oldthebibliography=\thebibliography
% %\let\oldendthebibliography=\endthebibliography
% %\renewenvironment{thebibliography}[1]{%
% %     \oldthebibliography{#1}%
% %     \setcounter{enumiv}{6}%
% %}{\oldendthebibliography}


% %%%%%%%%% PAPER ID  - PLEASE UPDATE
% \def\paperID{8798} % *** Enter the Paper ID here
% \def\confName{CVPR}
% \def\confYear{2023}

% \begin{document}

% %%%%%%%%% TITLE - PLEASE UPDATE
% \title{JRDB-PanoTrack: An Open-world Panoptic Segmentation and Tracking Robotic Dataset in Crowded Human Environments}  % **** Enter the paper title here

% \maketitle
% \thispagestyle{empty}
% \appendix

% %%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW
% %\noindent\textbf{#1 Dataset size (\Rone, \Rtwo).} #Tho verision
% We appreciate the reviewers for their efforts in the review. We summarize the questions into following sections.\\
% %# chenhui version
% \noindent\textbf{Dataset size (\Rone).} The primary purpose of JRDB-PanoTrack is to serve as a closed/open-world panoptic segmentation/tracking benchmark to evaluate the generalization capabilities of methods trained on larger datasets in open-world settings. JRDB-PanoTrack aims to provide a meaningful benchmark for these tasks to the intersection of computer vision and robotics. It's important to note that current benchmarks like MOT, KITTI, TAO, and TAO-OW are not necessarily large-scale in comparison. \\
% \noindent\textbf{Requirement of Extra Data (\Rone).} We refer \Rones to the response of Table 6. The aim of incorporation of external data is to show the knowledge transferabily between datasets.
% %The existing of such dataset to benchmark these task is lacking in the community %, many success benchmark KITTI MOT TAO may not necessarily large-scale and useful to train foundation models. our jrdb also serve the same purpose. even ours is small, in next section we demonstrate that our dataset has enough ....
% %The existing of such dataset to benchmark these task is lacking in the community, many success benchmark KITTI MOT TAO may not necessarily large-scale and useful to train foundation models. our jrdb also serve the same purpose. even ours is small, in next section we demonstrate that our dataset has enough ....

% % As a unique dataset captured on a robotic platform, our aim isn't a direct comparison with autonomous driving datasets but to offer extensive annotations valuable for the robotics community, enhancing understanding in dynamic environments.

% % We appreciate the feedback on our dataset's size. The primary goal of JRDB-PanoTrack is to serve as a benchmark, rather than training foundation models. The goal of JRDB-PanoTrack benchmark is to not just evaluate methods that were trained on the dataset, but also methods that were trained on massive datasets to see their generalisation when dealing with open-world settings. As one of the very limited datasets that was captured on robot platform, we are not comparing JRDB-PanoTrack directly with autonomous driving datasets, our extensive annotations suite is tailored for the robotics community, enhancing human understanding in dynamic environments.


% %addressing \Rtwo's concern.

% % Tho version \noindent\textbf{#2 Cross dataset generalisation (\Rone, \Rtwo).} We refer \Rone to the Tab. 6, which demonstrates knowledge transferability between datasets. We also show that the knowledge from JRDB-PanoTrack can help improve the performance when fine-tuning on COCO dataset (Table 9 in the supplementary) and vice-versa (Table 4). It suggests that the size of JRDB-PanoTrack does not significantly hinder the performance, addressing \Rtwo's concern. We apologise about the formatting issue in Tab. 6 and  will revise the table descriptions for better clarity. 

% \noindent\textbf{Scientific contribution (\Rtwo).}  In this paper, our main objective is to introduce a valuable benchmark to the computer vision and robotics fields. We focus on crafting high-quality, precisely tailored annotations, a process that involves significant teamwork and dedication. We believe this careful and detailed approach is fundamental and holds comparable values to the development of larger datasets with simpler annotations. Our aim is to deliver annotations that are not only of high quality but also specifically useful to the community, favoring in-depth and applicable insights over the data volume. Through this, we hope to make a meaningful and constructive contribution to the field.
% % \noindent\textbf{Multi-class segmentation (\Rtwo)} To facility object-to-object interaction understanding, JRDB-PanoTrack annotates multiple classes for some areas, such as the objects behind glass or being hang on wall. Our annotation process leverages the temporal context of video data, allowing for high-confidence labeling and avoiding hallucinations. This robust process, coupled with multiple quality checks, ensures annotation accuracy. Regarding evaluation on those multi-label areas, due to the fact that there is no available pretrained close/open-world panotic segmentation/tracking methods, we could not evaluate them in the multi-label settings, despite our proposed metrics are capable of. Specifically, we preprocess multi-label areas into a single-label setting (\textit{thing} objects are chosen if they are behind the class, and \textit{stuff} behind class is ignored) and use standard metrics for evaluation together with OSPA$_{PS}$ and OSPA$^{2}_{PT}$. We look forward for future methods that can fully utilise our dataset's multi-class segmentation capabilities.

% %\noindent\textbf{#3 Multi-class segmentation (\Rtwo).} JRDB-PanoTrack features multi-class annotations in specific areas, like objects behind glass or on walls, enhancing object interaction understanding. Our annotation process leverages the temporal context of video data, allowing for high-confidence labeling and avoiding hallucinations. Also, the absence of pretrained models for close/open-world panoptic segmentation/tracking limits our evaluation in multi-label settings. We preprocess these areas into single-label ones, selecting \textit{thing} objects and omitting \textit{stuff} behind them, to utilize standard evaluation metrics alongside OSPA$_{PS}$ and OSPA$^{2}_{PT}$. We hope future research can exploit the full potential of our dataset's multi-class segmentation annotations.

% \noindent\textbf{Annotation process (\Rtwo).} %Due to the significant scope and limited length of the paper, we could only provide limited details about our annotation process. 
% There are 3 senior annotators and several annotators. The annotation process starts with an unlimited list of classes which can be extended by all annotators, any clearly visible and semantically meaningful objects would be annotated. Then annotators produce labels and senior annotators control the quality by multiple rounds. We will provide more details in the revison.

% % \textcolor{red}{Please briefly introduce the process by 1 or 2 sentences.}%Also, we thank \Rthrees for pointing out the usage of the word "collected". We will revise accordingly.

% \noindent\textbf{Proposed metric (\Rtwo).} % As mentioned above, we also had to reduce the metric section. 
% For more clarification on OSPA$_{PS}$ and OSPA$^{2}_{PT}$, we would kindly refer \Rtwos to a recently published comprehensive study on the advantages of OSPA compared to other metrics [25]. %\textcolor{red}{Please briefly introduce the advantages (isn't it already mentioned in the paper?) (but the reviewer is hard to get. You goal is to make reviewers and ACs clear of your paper.)} %To briefly mention, OPSA
% To briefly introduce, current methods for panoptic segmentation heavily rely on PQ[16] , which is originally designed for single-label segmentation. %Our proposed metric, OSPA$_{PS}$ naturally supports multi-label panoptic segmentation. 
% %Our introduction of OSPA$_{PS}$ and OSPA$^{2}_{PT}$ is a natural extension of OSPA to panoptic segmentation and tracking. 
% OSPA-based metrics have several properties such as  multi-label capability, being non-threshold-based and not penalizing error correction. And we will add explanations of OSPA$_{PS}$ and OSPA$^{2}_{PT}$ in the final version. \\
% \noindent\textbf{3D label projection (\Rtwo).} We agree with \Rtwos that due to small miss-alignments, the projected 3D labels can't really be used as annotations for evaluations. That was why we did not claim and do many experiments on it. We have been actively improving the calibration and hopefully, these pseudo-annotations can be useful for methods that want to extend beyond 2D images. 

% \noindent\textbf{Evaluation settings (\Rtwo).} We apologize for any confusion regarding evaluation settings. To clarify, all models are trained and evaluated on individual camera views, compatible with most closed/open-world pretrained panoptic segmentation models. Since our track IDs are consistent across the camera views, we also provide the stitching script so that future research can project their prediction from individual to stitched view and run the evaluation. 

% \noindent\textbf{Multi-class segmentation (\Rtwo).} 
% % JRDB-PanoTrack features multi-class annotations in specific areas, like objects behind glass or on walls, enhancing object interaction understanding. 
% Our annotation process leverages the temporal context of video data, allowing for high-confidence labeling and avoiding hallucinations. Also, the absence of pretrained models for close/open-world panoptic segmentation/tracking limits our evaluation in multi-label settings. We preprocess these areas into single-label ones, selecting \textit{thing} objects and omitting \textit{stuff} behind them, to utilize standard evaluation metrics alongside OSPA$_{PS}$ and OSPA$^{2}_{PT}$. We hope future research can exploit the full potential of our dataset's multi-class segmentation annotations.



% % Given two sets of mask tracks of a class $c \in \mathbb{C}$, \ie $\mathbf{X_c}$ and $\mathbf{Y_c}$, we apply OSPA distance over time averaged distance $\widetilde{d}(X^{\mathcal{D}_i}_{ic}, Y^{\mathcal{D}_{\pi_i}}_{\pi_ic})$ of each pair of tracks 
% % $\mathcal{O}^2_{PT}&(\mathbf{X_c},\mathbf{Y_c})=\nonumber\\ \frac{1}{n}&\left(\min_{\pi \in \Pi_{n}} \sum_{i=1}^{m}\underline{\widetilde{d}}(X^{\mathcal{D}_i}_{ic}, Y^{\mathcal{D}_{\pi_i}}_{\pi_ic})+(n-m)\right)$.




% % To obtain the distance \ospapt \text{ }between two sets of mask tracks of a given class $c \in \mathbb{C}$, \ie $\mathbf{X_c}$ and $\mathbf{Y_c}$, we apply OSPA distance over time averaged distance $\widetilde{d}(X^{\mathcal{D}_i}_{ic}, Y^{\mathcal{D}_{\pi_i}}_{\pi_ic})$ of each pair of tracks 
% %     $\mathcal{O}^2_{PT}&(\mathbf{X_c},\mathbf{Y_c})=\nonumber\\ \frac{1}{n}&\left(\min_{\pi \in \Pi_{n}} \sum_{i=1}^{m}\underline{\widetilde{d}}(X^{\mathcal{D}_i}_{ic}, Y^{\mathcal{D}_{\pi_i}}_{\pi_ic})+(n-m)\right)$.
% % The Localization Error component $\min_{\pi \in \Pi_{n}} \sum_{i=1}^{m}\underline{\widetilde{d}}(X^{\mathcal{D}_i}_{ic}, Y^{\mathcal{D}_{\pi_i}}_{\pi_ic})$ will indirectly increase due to ID switches that cause poorer match and therefore a higher distance calculation. The second term, Cardinality Mismatch component $(n-m)$, primarily penalizes the difference in the number of tracks, it does not directly address ID switches. An ID switch doesn't necessarily change the number of tracks; it just mislabels them. Therefore, the cardinality mismatch part of the equation might not be sensitive to ID switches. This is one of the advantages of OSPA over IDF1 or MOTA, in which these metrics directly penalize ID switches, and inadvertently penalize the rectification of errors (ID recovery).


% \noindent\textbf{ID switch (\Rtwo).} Like the IDF1 metric, OSPA$^2$ implicitly handles ID switches, reflected in both localization and cardinality errors. ID switches lead to mismatches between predicted and ground truth (GT) tracks, increasing false tracks reflected in OSPA$^2$’s cardinality mismatch. Even minimal ID switches, where predicted tracks still match a GT track but under a different ID, would result in increased localization errors due to increased distances between matched tracks. Thus, OSPA$^2$ indirectly penalizes ID switches by affecting match quality and track count accuracy, offering a comprehensive evaluation of tracking performance. This approach contrasts with metrics directly penalizing ID switches, emphasizing OSPA$^2$’s nuanced evaluation strategy. 


% \label{Table6} \noindent \textbf{Table 6 (\Rone, \Rtwo)} demonstrates knowledge transferability between datasets in open-world setting. In the closed-world setting, we also show that the knowledge from JRDB-PanoTrack can help improve performance when fine-tuning on the COCO dataset (Table 9 in the supplementary) and vice versa (Table 4). The results in both open-world and closed-world settings show that using JRDB-PanoTrack improves segmentation performance in other domains. This suggests that the size of JRDB-PanoTrack does not significantly hinder the performance, addressing \Rtwo's concern. We apologize for the formatting issue in Table 6 and will revise the table.
% % Here is chenhui version
% % \noindent\textbf{Table 6 (\Rtwo).} 
% % Table 6 demonstrates knowledge transferability between datasets in the open-world setting. The knowledge from JRDB-PanoTrack can help COCO prediction, and vice versa. We apologize for the formatting issue in Table 6 and will revise the table for better clarity.
% % and layout for clarity in the final manuscript.

% %\noindent\textbf{#9 Scientific contribution emphasis (\Rone, \Rtwo).}: As this paper is not centered on methodology, our primary goal is to establish a meaningful benchmark for the computer vision and robotics communities. We emphasise the importance of creating high-quality, targeted annotations. This approach, we believe, is equally crucial as developing a large-scale dataset with basic annotations. Our commitment is to provide quality annotations that cater to the needs of the community, prioritizing meaningful insights over data volume.

% \noindent\textbf{`Collected' (\Rthree).} We change it to `employed'.

% \noindent\textbf{Image size in Fig. 4 (\Rtwo).} 752x480 (W x H).

% \noindent\textbf{Standard metrics (\Rthree).} %We thank \Rthrees for pointing this out. 
% We will add more descriptions and references, such as Panoptic Quality (PQ) [16] and Segmentation and Tracking Quality (STQ) [31], and other tracking metrics.
% %\textcolor{red}{briefly introduce or at least show the references.}

% %\noindent\textbf{#11 Writing corrections and extra information (\Rone, \Rtwo, \Rthree).} We thank the reviewers for noting the typos and the need for more detail. These issues will be thoroughly addressed in the final manuscript.

% % \small \vspace{-0.1cm}
% % \noindent
% % [Ref-A] Nguyen et al. \textit{How trustworthy are performance evaluations for basic
% % vision tasks?} IEEE TPAMI 2022


% %%%%%%%%% REFERENCES
% % {
% %     \small
% %     \bibliographystyle{ieeenat_fullname}
% %     \bibliography{main}
% % }

% \end{document}


==> sec/6_discussion.tex <==
\section{Discussion}

==> sec/tables/ablation.tex <==
% \begin{table*}[t]
% % \vspace{-.4cm}
%     \centering
%     %     \footnotesize
%     %         \renewcommand{\arraystretch}{1.6}
%     % \resizebox{\columnwidth}{!}{%
%     % \resizebox{\textwidth}{!}{%
%     \begin{adjustbox}{width=1.0\textwidth,center}
%     % \begin{tabular}{l|c|cccccc}
%     \begin{tabular}{l|ccc|ccc|ccc|}
%     \toprule
%     \multirow{2}{*}{Training Strategy} & 
%     \multicolumn{3}{c|}{All (43 classes)}&
%     \multicolumn{3}{c|}{Thing (32 classes)}&
%     \multicolumn{3}{c|}{Stuff (11 classes)}\\
%     \cmidrule(l{0pt}r{0pt}){2-10}
%      &PQ &SQ  & RQ &PQ$^{Th}$ &SQ$^{Th}$ & RQ$^{Th}$ &PQ$^{St}$&SQ$^{St}$  & RQ$^{St}$\\
%         \hline     
% Train from scratch & 21.37&69.35& 27.73 &16.80 & 66.95 & 21.80 &34.62 & 76.36 & 44.94\\
% Train from ImageNet & 31.41&79.13&39.44 &27.12 & 79.47 & 33.99 &43.88 & 78.16 & 55.29\\
% Train from COCO  & \textbf{36.56}&\textbf{81.08}&\textbf{44.98} &\textbf{33.06} & \textbf{81.47} & \textbf{40.56} &\textbf{46.73} & \textbf{79.97} & \textbf{57.85}\\
%         %Mask2Former & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
%         %Mask DINO & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
%         \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \centering
%     % \vspace{0.2cm}
%     \caption{Ablation study for different initialization strategies for MaskDino \cite{li2023mask} with a ResNet-50 backbone on JRDB panoptic close world test dataset.
%     % $\dag$ indicates the box AP is generated from mask prediction.
%     % $^*$ indicates it is the test-dev result.
%     % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
%     % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
%     }
    
%     \label{tab:panopti:initi}
%     \vspace{-.4cm}
% \end{table*}

\begin{table}[!tb]\centering
%\small
    %\begin{adjustbox}{width=0.5\textwidth,center}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l|cc|c|c|}
            \toprule
            
           % \multirow{2}{*}{Method} &
           % \multicolumn{2}{c|}{All (43 classes)} &
            %\multicolumn{2}{c|}{Thing (32 classes)}&
            %\multicolumn{2}{c|}{Stuff (11 classes)}\\
            %\multicolumn{3}{c|}{Mask Size} \\
           % \cmidrule(l{0pt}r{0pt}){2-5}
            Pretrain strategy & PQ  $\uparrow$     & \ospaps $\downarrow$   & \ospaps$^{Th}$   $\downarrow$ &\ospaps$^{St}$ $\downarrow$ \\
            \hline
            ImageNet \cite{deng2009imagenet}   & 31.41& 0.67&0.72& 0.53\\
            ImageNet \cite{deng2009imagenet} $\rightarrow$ COCO \cite{lin2014microsoft} & \textbf{36.57}&\textbf{0.63}&\textbf{0.68}&\textbf{0.51}\\
            \bottomrule
        \end{tabular}}
%}\end{adjustbox}
    \caption{We study how pretrain strategy affect the performance of MaskDino on JRDB panoptic close-world test dataset.}
    \label{tab:panoptic:ablation}
\end{table}

==> sec/tables/ablation16th_11.tex <==
\begin{table}[!tb]\centering
\small
    %\begin{adjustbox}{width=0.5\textwidth,center}
    \resizebox{ \linewidth}{!}{
   % \begin{adjustbox}{width=0.5\textwidth,center}
        \begin{tabular}{ll|cc|cc|cc}
            \toprule
            \multicolumn{2}{c|}{\textbf{Pretrain strategy}} &
            \multicolumn{2}{c|}{\textbf{All}} &
            \multicolumn{2}{c|}{\textbf{Thing}}&
            \multicolumn{2}{c}{\textbf{Stuff}}\\
           %\multicolumn{3}{c|}{Mask Size} \\
            \cmidrule(l{0pt}r{0pt}){1-8} 
             \textbf{ImageNet \cite{deng2009imagenet}} & \textbf{COCO }\cite{coco} & \textbf{PQ $\uparrow$}     & \textbf{\ospaps $\downarrow$}   &\textbf{PQ$^{Th}$ $\uparrow$}& \textbf{\ospaps$^{Th}$   $\downarrow$}  & \textbf{PQ$^{St}$$\uparrow$}&\textbf{\ospaps$^{St}$ $\downarrow$} \\ 
            \hline
            \textbf{\checkmark}&   & 31.41& 0.67& 27.12  & 0.72 &43.88 & 0.53\\
          \textbf{\checkmark}&\textbf{\checkmark}&\textbf{36.57}&\textbf{0.63} & 33.07 &\textbf{0.68}&46.74&\textbf{0.51}\\
            \bottomrule
         \end{tabular}}
            \caption{\small{We study how pretrain strategy affect the performance of MaskDino \cite{li2023mask} on JRDB-PanoTrack close-world test dataset. Two  strategies reported, pretraining with ImageNet only and pretraining with both ImageNet and COCO.}}
            %Note: We uses the official ResNet50 weights for inilizatizing the backbone of MaskDino \cite{li2023mask} }
    \label{tab:panoptic:ablation}
\end{table}

==> sec/tables/ablation_old.tex <==
% \begin{table*}[t]
% % \vspace{-.4cm}
%     \centering
%     %     \footnotesize
%     %         \renewcommand{\arraystretch}{1.6}
%     % \resizebox{\columnwidth}{!}{%
%     % \resizebox{\textwidth}{!}{%
%     \begin{adjustbox}{width=1.0\textwidth,center}
%     % \begin{tabular}{l|c|cccccc}
%     \begin{tabular}{l|ccc|ccc|ccc|}
%     \toprule
%     \multirow{2}{*}{Training Strategy} & 
%     \multicolumn{3}{c|}{All (43 classes)}&
%     \multicolumn{3}{c|}{Thing (32 classes)}&
%     \multicolumn{3}{c|}{Stuff (11 classes)}\\
%     \cmidrule(l{0pt}r{0pt}){2-10}
%      &PQ &SQ  & RQ &PQ$^{Th}$ &SQ$^{Th}$ & RQ$^{Th}$ &PQ$^{St}$&SQ$^{St}$  & RQ$^{St}$\\
%         \hline     
% Train from scratch & 21.37&69.35& 27.73 &16.80 & 66.95 & 21.80 &34.62 & 76.36 & 44.94\\
% Train from ImageNet & 31.41&79.13&39.44 &27.12 & 79.47 & 33.99 &43.88 & 78.16 & 55.29\\
% Train from COCO  & \textbf{36.56}&\textbf{81.08}&\textbf{44.98} &\textbf{33.06} & \textbf{81.47} & \textbf{40.56} &\textbf{46.73} & \textbf{79.97} & \textbf{57.85}\\
%         %Mask2Former & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
%         %Mask DINO & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
%         \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \centering
%     % \vspace{0.2cm}
%     \caption{Ablation study for different initialization strategies for MaskDino \cite{li2023mask} with a ResNet-50 backbone on JRDB panoptic close world test dataset.
%     % $\dag$ indicates the box AP is generated from mask prediction.
%     % $^*$ indicates it is the test-dev result.
%     % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
%     % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
%     }
    
%     \label{tab:panopti:initi}
%     \vspace{-.4cm}
% \end{table*}

\begin{table*}[t]
    \centering
    \begin{adjustbox}{width=1.0\textwidth,center}
    \begin{tabular}{l|cccc|cccc|cccc|}
    \toprule
    \multirow{2}{*}{Training Strategy} &
    \multicolumn{4}{c|}{All (43 classes)}&
    \multicolumn{4}{c|}{Thing (32 classes)}&
    \multicolumn{4}{c|}{Stuff (11 classes)}\\
    \cmidrule(l{0pt}r{0pt}){2-13}
     &PQ &SQ  & RQ &OSPA &PQ$^{Th}$ &SQ$^{Th}$ & RQ$^{Th}$ &OSPA$^{Th}$ &PQ$^{St}$&SQ$^{St}$  & RQ$^{St}$ &OSPA$^{St}$\\
        \hline
%Train from scratch & 21.37&69.35& 27.73 & [OSPA] &16.80 & 66.95 & 21.80 & [OSPA$^{Th}$] &34.62 & 76.36 & 44.94 & [OSPA$^{St}$]\\
Train from ImageNet & 31.41&79.13&39.44 & [OSPA] &27.12 & 79.47 & 33.99 & [OSPA$^{Th}$] &43.88 & 78.16 & 55.29 & [OSPA$^{St}$]\\
Train from COCO  & %\textbf{36.56}&\textbf{81.08}&\textbf{44.98} & [OSPA] &\textbf{33.06} & \textbf{81.47} & \textbf{40.56} & [OSPA$^{Th}$] &\textbf{46.73} & \textbf{79.97} & \textbf{57.85} & [OSPA$^{St}$]\\
\textbf{36.57}&\textbf{81.09}&\textbf{44.98} & [OSPA] &\textbf{33.07} & \textbf{81.47} & \textbf{40.56} & [OSPA$^{Th}$] &\textbf{46.74} & \textbf{79.98} & \textbf{57.85} & [OSPA$^{St}$]\\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Ablation study for different initialization strategies for MaskDino \cite{li2023mask} with a ResNet-50 backbone on JRDB panoptic close world test dataset.}
    \label{tab:panopti:initi}
\end{table*}

==> sec/tables/comparie_jrdb_image_on_COCO_old.tex <==
\begin{table*}[tb!]
% \vspace{-.4cm}
    \centering
    %     \footnotesize
    %         \renewcommand{\arraystretch}{1.6}
    % \resizebox{\columnwidth}{!}{%
    % \resizebox{\textwidth}{!}{%
    \begin{adjustbox}{width=1.0\textwidth,center}
    % \begin{tabular}{l|c|cccccc}
    \begin{tabular}{l|ccc|ccc|ccc|}
    \toprule
    \multirow{2}{*}{Method} & 
    \multicolumn{3}{c|}{All (133 classes)}&
    \multicolumn{3}{c|}{Thing (80 classes)}&
    \multicolumn{3}{c|}{Stuff (53 classes)}\\
    \cmidrule(l{0pt}r{0pt}){2-10}
     &PQ &SQ  & RQ &PQ$^{Th}$ &SQ$^{Th}$ & RQ$^{Th}$ &PQ$^{St}$&SQ$^{St}$  & RQ$^{St}$\\
        \hline     
ImageNet pretrain  & 42.16&80.11&50.39 &47.43 & 80.99 & 56.51 &34.20 & 78.78 & 41.15\\
JRDB pretrain  & \textbf{44.48} & \textbf{82.54}& \textbf{52.70} &\textbf{50.48} & \textbf{84.42} & \textbf{59.31} &\textbf{35.43} & \textbf{79.71} & \textbf{42.73}\\

        %Mask2Former & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
        %Mask DINO & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \centering
    \caption{Results between COCO-pretrained and JRDB-pretrained on COCO evaluation dataset using MaskDino with a ResNet-50 backbone.
    % $\dag$ indicates the box AP is generated from mask prediction.
    % $^*$ indicates it is the test-dev result.
    % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
    % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
    }
    
    \label{tab:panoptic}
\end{table*}

% \begin{table*}[tb!]
%     \centering
%     \begin{adjustbox}{width=1.0\textwidth,center}
%     \begin{tabular}{l|cccc|cccc|cccc|}
%     \toprule
%     \multirow{2}{*}{Method} &
%     \multicolumn{4}{c|}{All (133 classes)}&
%     \multicolumn{4}{c|}{Thing (80 classes)}&
%     \multicolumn{4}{c|}{Stuff (53 classes)}\\
%     \cmidrule(l{0pt}r{0pt}){2-13}
%      &PQ &SQ  & RQ &OSPA &PQ$^{Th}$ &SQ$^{Th}$ & RQ$^{Th}$ &OSPA$^{Th}$ &PQ$^{St}$&SQ$^{St}$  & RQ$^{St}$ &OSPA$^{St}$\\
%         \hline
% ImageNet pretrain *  & 42.16&80.11&50.39 &[OSPA] &47.43 & 80.99 & 56.51 &[OSPA$^{Th}$] &34.20 & 78.78 & 41.15 &[OSPA$^{St}$]\\
% JRDB pretrain& \textbf{44.48} & \textbf{82.54}& \textbf{52.70} &[OSPA] &\textbf{50.48} & \textbf{84.42} & \textbf{59.31} &[OSPA$^{Th}$] &\textbf{35.43} & \textbf{79.71} & \textbf{42.73} &[OSPA$^{St}$]\\
%         \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Results between COCO-pretrained and JRDB-pretrained on COCO evaluation dataset using MaskDino with a ResNet-50 backbone. * means wetrain this method under the same training strategy.}
%     \label{tab:jrdb_on_coco}



==> sec/tables/jrdb_help_coco_old.tex <==

%%% results update 

\begin{table}[!tb]
\small
\centering
\resizebox{\linewidth}{!}{
% \vspace{-.4cm}
    
    %     \footnotesize
    %         \renewcommand{\arraystretch}{1.6}
    % \resizebox{\columnwidth}{!}{%
    % \resizebox{\textwidth}{!}{%
    %\begin{adjustbox}{width=1.0\textwidth,center}
    % \begin{tabular}{l|c|cccccc}
    \begin{tabular}{l|cc|}
    \toprule
   
    %Method& COCO &JRDB-PanoTrack \\
   \multirow{2}{*}{Train data} & 
   \multicolumn{2}{c|}{Test data}\\
   \cmidrule{2-3}
  %  \multicolumn{3}{c|}{JRDB-PanoTrack(71 classes)}\\
   % \cmidrule(l{0pt}r{4pt}){2-3}\\
     & COCO evl &JRDB-PanoTrack \\
     \hline
%COCO $\rightarrow$ JRDB & 10.08&50.76&12.57 & - & -& -\\
%JRDB $\rightarrow$ COCO & -&-&- &13.70& 73.05 & 17.75\\
%FreeSeg (no pretrained model)   & && & & & &&  & \\
COCO Train  &- & 10.08 PQ\\
JRDB-PanoTrack Train & 13.70 PQ &-\\
        %Mask2Former & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
        %Mask DINO & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
        \bottomrule
    \end{tabular}}
   % \end{adjustbox}
    \centering
    % \vspace{0.2cm}
    \caption{Results for FC-CLIP \cite{yu2023convolutions} trained with different training data and do zero-shot inference on other dataset.}
    
    % $\dag$ indicates the box AP is generated from mask prediction.
    % $^*$ indicates it is the test-dev result.
    % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
    % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
    
    
    \label{tab:panoptic_jrdb_helpcoco}
\end{table}

==> sec/tables/panopticSeg_All_in_one.tex <==
\begin{table*}[!htp]\centering
% \vspace{-.4cm}
    \centering
    %     \footnotesize
    %         \renewcommand{\arraystretch}{1.6}
    % \resizebox{\columnwidth}{!}{%
    % \resizebox{\textwidth}{!}{%
    \begin{adjustbox}{width=1.0\textwidth,center}
    % \begin{tabular}{l|c|cccccc}
    \begin{tabular}{l|ccc|ccc|ccc|ccc|}
    \toprule
    \multirow{2}{*}{Method} & 
    \multicolumn{3}{c|}{Common ($43$ classes)}&
    \multicolumn{3}{c|}{Hidden ($28$ classes)}&
    \multicolumn{3}{c|}{Known ($20$ classes)}&
    \multicolumn{3}{c|}{Unknown ($51$ classes)}\\
    \cmidrule(l{0pt}r{0pt}){2-13}
    & PQ$^{C}$ &SQ$^{C}$ & RQ$^{C}$ &PQ$^{H}$&SQ$^{H}$  & RQ$^{H}$ &PQ$^{K}$ &SQ$^{K}$ & RQ$^{K}$ &PQ$^{U}$&SQ$^{U}$  & RQ$^{U}$\\
        \hline
%FC-CLIP \textcolor{red}{Current Sota} & $12.97$&$56.81$&$16.02$ &$8.38$ & $52.16$ & $10.25$ &$26.32$ & $70.34$ & $32.80$\\


ODISE \cite{xu2023open} &\textbf{14.94}&65.80 &\textbf{18.69} &3.86& 42.47&4.69 &\textbf{24.35}&\textbf{78.56} &\textbf{30.62} &5.17& 48.00&6.33 \\
ODISE \cite{xu2023open} (caption)  & 13.58 &\textbf{68.64} & 16.79 &\textbf{7.18}& \textbf{50.67}& \textbf{8.75} & 22.27 &70.50 & 27.51 &\textbf{6.66}& \textbf{58.04}& \textbf{8.18}\\
FC-CLIP \cite{yu2023convolutions} &$14.29$ & $58.98$ & $17.89$ &$3.62$ & $38.15$ & $4.41$ &24.09 & 78.25 & 30.28 &4.60 & 39.98 & 5.63\\

MaskClip & && & & & &&  & & &\\
        %Mask2Former & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
        %Mask DINO & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \centering
    % \vspace{0.2cm}
    \caption{Results for current sota open world panoptic segmentation models on JRDB test dataset. There are $71$ classes in the JRDB open-world test dataset. $43$ classes are all used in a closed world, described as Common classes, $28$ classes are hidden in a JRDB close-world test dataset. described as Hidden classes.
    % $\dag$ indicates the box AP is generated from mask prediction.
    % $^*$ indicates it is the test-dev result.
    % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
    % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
    }
    
    \label{tab:panoptic_common_hidden}
\end{table*}

==> sec/tables/panopticSeg_Common_Hidden.tex <==
\begin{table*}[!tb]\centering
% \vspace{-.4cm}
    \centering
    %     \footnotesize
    %         \renewcommand{\arraystretch}{1.6}
    % \resizebox{\columnwidth}{!}{%
    % \resizebox{\textwidth}{!}{%
    \begin{adjustbox}{width=1.0\textwidth,center}
    % \begin{tabular}{l|c|cccccc}
    \begin{tabular}{l|ccc|ccc|ccc|}
    \toprule
    \multirow{2}{*}{Method} & 
    \multicolumn{3}{c|}{All ($71$ classes)}&
    \multicolumn{3}{c|}{Common ($43$ classes)}&
    \multicolumn{3}{c|}{Hidden ($28$ classes)}\\
    \cmidrule(l{0pt}r{0pt}){2-10}
     &PQ &SQ  & RQ &PQ &SQ & RQ &PQ&SQ  & RQ\\
        \hline
%FC-CLIP \textcolor{red}{Current Sota} & $12.97$&$56.81$&$16.02$ &$8.38$ & $52.16$ & $10.25$ &$26.32$ & $70.34$ & $32.80$\\


ODISE \cite{xu2023open} &10.57 &56.60&13.17 &\textbf{14.94}&65.80 &\textbf{18.69} &3.86& 42.47&4.69\\
ODISE \cite{xu2023open} (caption) & \textbf{11.06}&\textbf{61.55}& \textbf{13.62} & 13.58 &\textbf{68.64} & 16.79 &\textbf{7.18}& \textbf{50.67}& \textbf{8.75}\\
FC-CLIP \cite{yu2023convolutions} & $10.09$&$50.76$&$12.57$ &$14.29$ & $58.98$ & $17.89$ &$3.62$ & $38.15$ & $4.41$\\
FC-CLIP  \cite{yu2023convolutions} $\dotplus$ & 16.37&62.95&20.15 &24.95 & 78.21 & 30.91 &3.19 & 39.52 & 3.63\\

%MaskClip & && & & & &&  & \\
        %Mask2Former & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
        %Mask DINO & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \centering
    % \vspace{0.2cm}
    \caption{Results for current sota open world panoptic segmentation models on JRDB test dataset. There are $71$ classes in the JRDB open-world test dataset. $43$ classes are all used in a closed world, described as Frequent classes, $28$ classes are hidden in a JRDB close-world test dataset. described as Long-tail classes.
    % $\dag$ indicates the box AP is generated from mask prediction.
    % $^*$ indicates it is the test-dev result.
    % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
    % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
    }
    
    \label{tab:panoptic_common_hidden}
\end{table*}

==> sec/tables/panopticSeg_close_world.tex <==
% \begin{table*}[t]
% % \vspace{-.4cm}
%     \centering
%     %     \footnotesize
%     %         \renewcommand{\arraystretch}{1.6}
%     % \resizebox{\columnwidth}{!}{%
%     % \resizebox{\textwidth}{!}{%
%     \begin{adjustbox}{width=1.0\textwidth,center}
%     % \begin{tabular}{l|c|cccccc}
%     \begin{tabular}{l|ccc|ccc|ccc|}
%     \toprule
%     \multirow{2}{*}{Method} & 
%     \multicolumn{3}{c|}{All (43 classes)}&
%     \multicolumn{3}{c|}{Thing (32 classes)}&
%     \multicolumn{3}{c|}{Stuff (11 classes)}\\
%     \cmidrule(l{0pt}r{0pt}){2-10}
%      &PQ &SQ  & RQ &PQ$^{Th}$ &SQ$^{Th}$ & RQ$^{Th}$ &PQ$^{St}$&SQ$^{St}$  & RQ$^{St}$\\
%         \hline     
% kMaX-DeepLab \cite{yu2022k} & 32.52&77.78&41.38 &27.96 & 77.23 & 36.00 &45.81 & 79.38 & 57.04\\
% Mask2Former \cite{cheng2021mask2former} & 33.24&80.55&41.33 &28.72 & 80.83 & 35.77 &46.38 & 79.74 & 57.51\\
% Mask DINO \cite{li2023mask} & \textbf{36.56}&\textbf{81.08}&\textbf{44.98} &\textbf{33.06} & \textbf{81.47} & \textbf{40.56} &\textbf{46.73} & \textbf{79.97} & \textbf{57.85}\\
%         %Mask2Former & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
%         %Mask DINO & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
%         \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \centering
%     % \vspace{0.2cm}
%     \caption{Results for panoptic segmentation models (COCO-pretrained) with a ResNet-50 backbone on JRDB panoptic close-world test dataset.
%     % $\dag$ indicates the box AP is generated from mask prediction.
%     % $^*$ indicates it is the test-dev result.
%     % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
%     % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
%     }
    
%     \label{tab:panoptic:closeworld}
%     \vspace{-.4cm}
% \end{table*}
%




%% close world result update : chenhui 11th 11.
% \begin{table*}[t]
%     \centering
%     \begin{adjustbox}{width=1.0\textwidth,center}
%     \begin{tabular}{l|cccc|cccc|cccc|}
%     \toprule
%     \multirow{2}{*}{Method} &
%     \multicolumn{4}{c|}{All (43 classes)}&
%     \multicolumn{4}{c|}{Thing (32 classes)}&
%     \multicolumn{4}{c|}{Stuff (11 classes)}\\
%     \cmidrule(l{0pt}r{0pt}){2-13}
%      &PQ &SQ  & RQ & OSPA &PQ$^{Th}$ &SQ$^{Th}$ & RQ$^{Th}$ & OSPA$^{Th}$ &PQ$^{St}$&SQ$^{St}$  & RQ$^{St}$ & OSPA$^{St}$\\
%         \hline
% kMaX-DeepLab \cite{yu2022k} & 32.52&77.78&41.38 & [OSPA] &27.96 & 77.23 & 36.00 & [OSPA$^{Th}$] &45.81 & 79.38 & 57.04 & [OSPA$^{St}$]\\
% Mask2Former \cite{cheng2021mask2former} & 33.25&80.53&41.35 & [OSPA] &28.74 & 80.81 & 35.79 & [OSPA$^{Th}$] &46.38 & 79.73 & 57.51 & [OSPA$^{St}$]\\
% Mask DINO \cite{li2023mask} & \textbf{36.57}&\textbf{81.09}&\textbf{44.98} & [OSPA] &\textbf{33.07} & \textbf{81.47} & \textbf{40.56} & [OSPA$^{Th}$] &\textbf{46.74} & \textbf{79.98} & \textbf{57.85} & [OSPA$^{St}$]\\
%         \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Results for panoptic segmentation models (COCO-pretrained) with a ResNet-50 backbone on JRDB panoptic close-world test dataset.}
%     \label{tab:panoptic:closeworld}
% \end{table*}

\begin{table}[!tb]\centering
%\small
    %\begin{adjustbox}{width=0.5\textwidth,center}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l|cc|c|c|}
            \toprule
            
           % \multirow{2}{*}{Method} &
           % \multicolumn{2}{c|}{All (43 classes)} &
            %\multicolumn{2}{c|}{Thing (32 classes)}&
            %\multicolumn{2}{c|}{Stuff (11 classes)}\\
            %\multicolumn{3}{c|}{Mask Size} \\
           % \cmidrule(l{0pt}r{0pt}){2-5}
            Method & PQ  $\uparrow$     & \ospaps $\downarrow$   & \ospaps$^{Th}$   $\downarrow$ &\ospaps$^{St}$ $\downarrow$ \\
            \hline
            kMaX-DeepLab \cite{yu2022k}   & 32.52& 0.67&0.72& 0.53\\
            Mask2Former \cite{cheng2021mask2former} & 33.25&0.66&0.71&0.52\\
            Mask DINO \cite{li2023mask} & \textbf{36.57}&\textbf{0.63}&\textbf{0.68}&\textbf{0.51}\\
            \bottomrule
        \end{tabular}}
%}\end{adjustbox}
    \caption{Results for panoptic segmentation models (COCO-pretrained) with a ResNet-50 backbone on JRDB-PanoTrack close-world test dataset.}
    \label{tab:panoptic:closeworld}
\end{table}

==> sec/tables/panopticSeg_close_world_old.tex <==
% \begin{table*}[t]
% % \vspace{-.4cm}
%     \centering
%     %     \footnotesize
%     %         \renewcommand{\arraystretch}{1.6}
%     % \resizebox{\columnwidth}{!}{%
%     % \resizebox{\textwidth}{!}{%
%     \begin{adjustbox}{width=1.0\textwidth,center}
%     % \begin{tabular}{l|c|cccccc}
%     \begin{tabular}{l|ccc|ccc|ccc|}
%     \toprule
%     \multirow{2}{*}{Method} & 
%     \multicolumn{3}{c|}{All (43 classes)}&
%     \multicolumn{3}{c|}{Thing (32 classes)}&
%     \multicolumn{3}{c|}{Stuff (11 classes)}\\
%     \cmidrule(l{0pt}r{0pt}){2-10}
%      &PQ &SQ  & RQ &PQ$^{Th}$ &SQ$^{Th}$ & RQ$^{Th}$ &PQ$^{St}$&SQ$^{St}$  & RQ$^{St}$\\
%         \hline     
% kMaX-DeepLab \cite{yu2022k} & 32.52&77.78&41.38 &27.96 & 77.23 & 36.00 &45.81 & 79.38 & 57.04\\
% Mask2Former \cite{cheng2021mask2former} & 33.24&80.55&41.33 &28.72 & 80.83 & 35.77 &46.38 & 79.74 & 57.51\\
% Mask DINO \cite{li2023mask} & \textbf{36.56}&\textbf{81.08}&\textbf{44.98} &\textbf{33.06} & \textbf{81.47} & \textbf{40.56} &\textbf{46.73} & \textbf{79.97} & \textbf{57.85}\\
%         %Mask2Former & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
%         %Mask DINO & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
%         \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \centering
%     % \vspace{0.2cm}
%     \caption{Results for panoptic segmentation models (COCO-pretrained) with a ResNet-50 backbone on JRDB panoptic close-world test dataset.
%     % $\dag$ indicates the box AP is generated from mask prediction.
%     % $^*$ indicates it is the test-dev result.
%     % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
%     % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
%     }
    
%     \label{tab:panoptic:closeworld}
%     \vspace{-.4cm}
% \end{table*}
%




%% close world result update : chenhui 11th 11.
% \begin{table*}[t]
%     \centering
%     \begin{adjustbox}{width=1.0\textwidth,center}
%     \begin{tabular}{l|cccc|cccc|cccc|}
%     \toprule
%     \multirow{2}{*}{Method} &
%     \multicolumn{4}{c|}{All (43 classes)}&
%     \multicolumn{4}{c|}{Thing (32 classes)}&
%     \multicolumn{4}{c|}{Stuff (11 classes)}\\
%     \cmidrule(l{0pt}r{0pt}){2-13}
%      &PQ &SQ  & RQ & OSPA &PQ$^{Th}$ &SQ$^{Th}$ & RQ$^{Th}$ & OSPA$^{Th}$ &PQ$^{St}$&SQ$^{St}$  & RQ$^{St}$ & OSPA$^{St}$\\
%         \hline
% kMaX-DeepLab \cite{yu2022k} & 32.52&77.78&41.38 & [OSPA] &27.96 & 77.23 & 36.00 & [OSPA$^{Th}$] &45.81 & 79.38 & 57.04 & [OSPA$^{St}$]\\
% Mask2Former \cite{cheng2021mask2former} & 33.25&80.53&41.35 & [OSPA] &28.74 & 80.81 & 35.79 & [OSPA$^{Th}$] &46.38 & 79.73 & 57.51 & [OSPA$^{St}$]\\
% Mask DINO \cite{li2023mask} & \textbf{36.57}&\textbf{81.09}&\textbf{44.98} & [OSPA] &\textbf{33.07} & \textbf{81.47} & \textbf{40.56} & [OSPA$^{Th}$] &\textbf{46.74} & \textbf{79.98} & \textbf{57.85} & [OSPA$^{St}$]\\
%         \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Results for panoptic segmentation models (COCO-pretrained) with a ResNet-50 backbone on JRDB panoptic close-world test dataset.}
%     \label{tab:panoptic:closeworld}
% \end{table*}

\begin{table*}[t]
    \centering
    \begin{adjustbox}{width=1.0\textwidth,center}
        \begin{tabular}{l|cccc|cccc|cccc|ccc|}
            \toprule
            \multirow{2}{*}{Method} &
            \multicolumn{4}{c|}{All (43 classes)} &
            \multicolumn{4}{c|}{Thing (32 classes)}&
            \multicolumn{4}{c|}{Stuff (11 classes)}&
            \multicolumn{3}{c|}{Mask Size} \\
            \cmidrule(l{0pt}r{0pt}){2-16}
            & PQ             & SQ             & RQ             & OSPA   & PQ$^{Th}$      & SQ$^{Th}$      & RQ$^{Th}$      & OSPA$^{Th}$   & PQ$^{St}$      & SQ$^{St}$      & RQ$^{St}$ & OSPA$^{St}$ & Small & Medium & Large\\
            \hline
            kMaX-DeepLab \cite{yu2022k}             & 32.52          & 77.78          & 41.38          & [OSPA] & 27.96          & 77.23          & 36.00          & [OSPA$^{Th}$] & 45.81 & 79.38 & 57.04 & [OSPA$^{St}$] & & & \\
            Mask2Former \cite{cheng2021mask2former} & 33.25          & 80.53          & 41.35          & 0.655 & 28.74          & 80.81          & 35.79 & 0.705 & 46.38 & 79.73 & 57.51 & 0.520 &0.804 & 0.589 & 0.371\\
            Mask DINO \cite{li2023mask}             & \textbf{36.57} & \textbf{81.09} & \textbf{44.98} & 0.635  & \textbf{33.07} & \textbf{81.47} & \textbf{40.56} & 0.683 & \textbf{46.74} & \textbf{79.98} & \textbf{57.85} & 0.513 & 0.785 & 0.552 & 0.364\\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
    \caption{Results for panoptic segmentation models (COCO-pretrained) with a ResNet-50 backbone on JRDB panoptic close-world test dataset.}
    \label{tab:panoptic:closeworld}
\end{table*}

==> sec/tables/panopticSeg_known_unknow.tex <==
\begin{table*}[!htp]
% \vspace{-.4cm}
    \centering
    %     \footnotesize
    %         \renewcommand{\arraystretch}{1.6}
    % \resizebox{\columnwidth}{!}{%
    % \resizebox{\textwidth}{!}{%
    \begin{adjustbox}{width=1.0\textwidth,center}
    % \begin{tabular}{l|c|cccccc}
    \begin{tabular}{l|ccc|ccc|ccc|}
    \toprule
    \multirow{2}{*}{Method} & 
    \multicolumn{3}{c|}{All ($71$ classes)}&
    \multicolumn{3}{c|}{Known ($20$ classes)}&
    \multicolumn{3}{c|}{Unknown ($51$ classes)}\\
    \cmidrule(l{0pt}r{0pt}){2-10}
     &PQ &SQ  & RQ &PQ &SQ& RQ &PQ&SQ  & RQ\\
        \hline
%FC-CLIP \textcolor{red}{Current Sota} & $12.97$&$56.81$&$16.02$ &$8.38$ & $52.16$ & $10.25$ &$26.32$ & $70.34$ & $32.80$\\


ODISE \cite{xu2023open} &10.57 &56.60&13.17 &\textbf{24.35}&\textbf{78.56} &\textbf{30.62} &5.17& 48.00&6.33\\
ODISE \cite{xu2023open} (caption) & \textbf{11.06}&\textbf{61.55}& \textbf{13.62}& 22.27 &70.50 & 27.51 &\textbf{6.66}& \textbf{58.04}& \textbf{8.18}\\
FC-CLIP \cite{yu2023convolutions}& 10.09&50.76&12.57 &24.09 & 78.25 & 30.28 &4.60 & 39.98 & 5.63\\

FC-CLIP  \cite{yu2023convolutions} $\dotplus$ & 16.37&62.95&20.15 &27.12 & 71.90 & 33.45 &12.15 & 59.45 & 14.94\\
        %Mask2Former & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
        %Mask DINO & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \centering
    \caption{Results for current sota open world panoptic segmentation models on JRDB test dataset. There are $71$ classes in the JRDB open-world test dataset. $20$ classes exist in COCO panoptic dataset \cite{lin2014microsoft}, denoted as Known classes, the left $51$ classes denoted as Unknown classes.
    % $\dag$ indicates the box AP is generated from mask prediction.
    % $^*$ indicates it is the test-dev result.
    % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
    % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
    }
    
    \label{tab:panoptic_known_unknown}
\end{table*}

==> sec/tables/panopticSeg_known_unknow_cross_indomain.tex <==
% \begin{table*}[!tb]
% % \vspace{-.4cm}
% \scriptsize
%     \centering
%     %     \footnotesize
%              \renewcommand{\arraystretch}{1.5}
%     % \resizebox{\columnwidth}{!}{%
%     \resizebox{\textwidth}{!}{%
%     %\begin{adjustbox}{width=1\textwidth,center}
%     % \begin{tabular}{l|c|cccccc}
%     %\resizebox{1.0\linewidth}{!}{
%     \begin{tabular}{l|l|cccccc|cc}
%     \toprule%\multicolumn{2}{c|}{All (43 classes)} &
%     \multirow{3}{*}{\textbf{Domain}} &\multirow{3}{*}{\textbf{ Method}} & \multicolumn{6}{c|}{\textbf{Known}} &\multicolumn{2}{c}{\textbf{Unknown}}\\
%     \cmidrule(l{0pt}r{0pt}){3-10} 
%     & & \multicolumn{2}{c}{\textbf{All}}& \multicolumn{2}{c}{\textbf{Thing}} &\multicolumn{2}{c|}{\textbf{Stuff}} & \multicolumn{2}{c}{\textbf{All/Thing}}\\%&\multicolumn{2}{c}{Thing} &\multicolumn{2}{c}{Stuff}\\
%     %\cmidrule(l{0pt}r{0pt}){3-10} \\
%     \cmidrule(l{0pt}r{0pt}){3-10}
%     &&  \textbf{PQ$\uparrow$} & \textbf{\ospaps$\downarrow$} &\textbf{PQ$^{Th}$ $\uparrow$} & \textbf{\ospaps$^{Th}$ $\downarrow$} & \textbf{PQ$^{St}$ $\uparrow$} & \textbf{\ospaps$^{St}$ $\downarrow$} &\textbf{PQ$\uparrow$} &\textbf{\ospaps $\downarrow$}\\
    
%    % & \ospaptboldu $\downarrow$ & PQ$^{Th}$ $\uparrow$ & \ospapt $\downarrow$ & PQ$^{St}$ $\uparrow$ & \ospaps $\downarrow$\\
%     %\cmidrule(l{0pt}r{0pt}){3-8} 
%     \hline
%     %\multicolumn{3}{c}{Cross-Domain}& & & & & & & & & \\
%    %& & & & & & & & & \\
%    \multirow{3}{*}{\textbf{Cross Domain}} 
%    & \textbf{ODISE} \cite{xu2023open}&14.94& 0.84 &9.80 &0.89 & 29.87  &0.72 & 3.86&\textbf{0.92}\\
%    &  \textbf{ODISE} \cite{xu2023open}(caption) &13.58& 0.84 &9.47 & 0.87&25.55 &0.78  &\textbf{7.18} & \textbf{0.92}\\
%    %& \textbf{FC-CLIP} \cite{yu2023convolutions} &14.29 & 0.86 & 10.18&0.89  & 26.43&0.78&3.62 &0.93\\
%    & \textbf{FC-CLIP} \cite{yu2023convolutions} &14.29 & 0.86 & 10.14&0.89  & 26.36&0.78&3.56 &0.93\\
%    \hline
%   \textbf{In Domain} & \textbf{FC-CLIP $\dotplus$} \cite{yu2023convolutions} &\textbf{24.95} & \textbf{0.75} &21.18 &\textbf{0.78}  & \textbf{35.94}&\textbf{0.69} &3.19 &0.98\\
%   %   &FC-CLIP \cite{yu2023convolutions} &14.29 &3.62  & & \\
     
%     %\cmidrule(l{0pt}r{0pt}){2-10}
%      %&PQ &SQ  & RQ &PQ &SQ& RQ &PQ&SQ  & RQ\\
%         %In Domain &FC-CLIP  \cite{yu2023convolutions} $\dotplus$ &\textbf{27.12} &\textbf{12.15}\\
%      %   In Domain &FC-CLIP  \cite{yu2023convolutions} $\dotplus$ &\textbf{24.95} &3.19 & & \\
% %FC-CLIP \textcolor{red}{Current Sota} & $12.97$&$56.81$&$16.02$ &$8.38$ & $52.16$ & $10.25$ &$26.32$ & $70.34$ & $32.80$\\


%         %Mask2Former & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
%         %Mask DINO & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
%         \bottomrule
%     %\multicolumn{2}{c|}{ Known (PQ)} &
%     %\multicolumn{2}{c|Unknown (PQ)} \\

%         \end{tabular}}
    
%     \centering
%     % \vspace{0.2cm}
%     \caption{
%     \scriptsize\textbf{We present the performance of state-of-the-art open world panoptic segmentation models on the JRDB Known-Unknown benchmark.} In the 'Cross Domain' evaluation, models pretrained on the COCO dataset are used for zero-shot inference on JRDB. For the 'In Domain' evaluation, models are trained on the JRDB training set and then tested on the JRDB-Panotrack open vocabulary test set. Here, 'Known' classes are defined as the 43 classes shared between the training and test sets, while 'Unknown' classes are those unique to the JRDB-Panotrack test set. Note: All 'Unknown' classes are 'Thing' classes. $\dotplus$ means we train this model by ourself only on JRDB-Panotrack training dataset without extra COCO pretrained.}
    
%     %Results for current sota open world panoptic segmentation models on JRDB Known-Unknown benchmark. For "Cross Domain" evaluation, we use coco-pretrained model and zero shot inference on JRDB, the Known classes would the shared classes between COCO and JRDB Panotrack, 20 classes are shared, left 51 are unknow classes. For "In Domain" evaluation, the model is trained on JRDB training set and  inference on JRDB test-set. The known classed would be the shared classes between JRDB training set and JRDB test-set, 43 classes are Known, left 28 are Unknown classes.
%  %Here, 'Known' classes are the 20 overlapping classes between COCO and JRDB Panotrack, with the remaining 51 classes categorized as 'Unknown'.
%     %Performance of current leading open world panoptic segmentation models on the JRDB Known-Unknown benchmark is presented. In the 'Cross Domain' evaluation, we employ models pretrained on COCO, performing zero-shot inference on JRDB.
%     %For the 'In Domain' evaluation, models are trained on the JRDB training set and tested on the JRDB-Panotrack open vocabulary test set. We define the Known classes contains 43 shared classes between the training and test sets. The Unknown classes are the classes only occurs in JRDB-Panotrack test set.
%     % $\dag$ indicates the box AP is generated from mask prediction.
%     % $^*$ indicates it is the test-dev result.
%     % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
%     % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
    
   
%     \label{tab:panopticSeg_known_unknow_cross_indomain}

% \end{table*}


\begin{table*}[!tb]
\small
\centering
\begin{adjustbox}{width=\textwidth, center}
    \begin{tabular}{l|l|cccccc|cc}
    \toprule
    \multirow{2}{*}{\textbf{Domain}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{6}{c|}{\textbf{Known}} & \multicolumn{2}{c}{\textbf{Unknown}}\\
    \cmidrule(l{0pt}r{0pt}){3-10} 
    &&  \textbf{PQ$\uparrow$} & \textbf{\ospapsbold$\downarrow$} & \textbf{PQ$^{\textbf{Th}}$ $\uparrow$} & \textbf{\ospapsboldt$\downarrow$} & \textbf{PQ$^{\textbf{St}}$ $\uparrow$} & \textbf{\ospapsbolds$\downarrow$} & \textbf{PQ$\uparrow$} & \textbf{\ospapsbold$\downarrow$}\\\midrule
    \multirow{3}{*}{\textbf{Cross-Domain}} 
    & \textbf{ODISE-L}\cite{xu2023open}&14.94& 0.84 &9.80 &0.89 & 29.87  &0.72 & 3.86&\textbf{0.92}\\
    &  \textbf{ODISE-C}\cite{xu2023open} &13.58& 0.84 &9.47 & 0.87&25.55 &0.78  &\textbf{7.18} & \textbf{0.92}\\
    & \textbf{FC-CLIP}\cite{yu2023convolutions} &14.29 & 0.86 & 10.14&0.89  & 26.36&0.78&3.56 &0.93\\\midrule
    \textbf{In-Domain} & \textbf{FC-CLIP$\dotplus$}\cite{yu2023convolutions} &\textbf{24.95} & \textbf{0.75} &21.18 &\textbf{0.78}  & \textbf{35.94}&\textbf{0.69} &3.19 &0.98\\
    \bottomrule
    \end{tabular}
\end{adjustbox}
\caption{\scriptsize\textbf{Performance of SOTA OW panoptic segmentation models on JRDB-PanoTrack.} Cross-domain methods are trained on COCO and tested on our dataset, while in-domain methods are trained with JRDB-PanoTrack \textit{known} classes. ODISE-L and ODISE-C represent ODISE results with label and caption prompts, respectively.}
\label{tab:panopticSeg_known_unknow_cross_indomain}
\end{table*}



==> sec/tables/panoptic_open_world_71.tex <==
% \begin{table*}[t]
% % \vspace{-.4cm}
%     \centering
%     %     \footnotesize
%     %         \renewcommand{\arraystretch}{1.6}
%     % \resizebox{\columnwidth}{!}{%
%     % \resizebox{\textwidth}{!}{%
%     \begin{adjustbox}{width=1.0\textwidth,center}
%     % \begin{tabular}{l|c|cccccc}
%     \begin{tabular}{l|ccc|ccc|ccc|}
%     \toprule
%     \multirow{2}{*}{Method} & 
%     \multicolumn{3}{c|}{All (43 classes)}&
%     \multicolumn{3}{c|}{Thing (32 classes)}&
%     \multicolumn{3}{c|}{Stuff (11 classes)}\\
%     \cmidrule(l{0pt}r{0pt}){2-10}
%      &PQ &SQ  & RQ &PQ$^{Th}$ &SQ$^{Th}$ & RQ$^{Th}$ &PQ$^{St}$&SQ$^{St}$  & RQ$^{St}$\\
%         \hline     
% kMaX-DeepLab \cite{yu2022k} & 32.52&77.78&41.38 &27.96 & 77.23 & 36.00 &45.81 & 79.38 & 57.04\\
% Mask2Former \cite{cheng2021mask2former} & 33.24&80.55&41.33 &28.72 & 80.83 & 35.77 &46.38 & 79.74 & 57.51\\
% Mask DINO \cite{li2023mask} & \textbf{36.56}&\textbf{81.08}&\textbf{44.98} &\textbf{33.06} & \textbf{81.47} & \textbf{40.56} &\textbf{46.73} & \textbf{79.97} & \textbf{57.85}\\
%         %Mask2Former & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
%         %Mask DINO & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
%         \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \centering
%     % \vspace{0.2cm}
%     \caption{Results for panoptic segmentation models (COCO-pretrained) with a ResNet-50 backbone on JRDB panoptic close-world test dataset.
%     % $\dag$ indicates the box AP is generated from mask prediction.
%     % $^*$ indicates it is the test-dev result.
%     % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
%     % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
%     }
    
%     \label{tab:panoptic:closeworld}
%     \vspace{-.4cm}
% \end{table*}
%




%% close world result update : chenhui 11th 11.
% \begin{table*}[t]
%     \centering
%     \begin{adjustbox}{width=1.0\textwidth,center}
%     \begin{tabular}{l|cccc|cccc|cccc|}
%     \toprule
%     \multirow{2}{*}{Method} &
%     \multicolumn{4}{c|}{All (43 classes)}&
%     \multicolumn{4}{c|}{Thing (32 classes)}&
%     \multicolumn{4}{c|}{Stuff (11 classes)}\\
%     \cmidrule(l{0pt}r{0pt}){2-13}
%      &PQ &SQ  & RQ & OSPA &PQ$^{Th}$ &SQ$^{Th}$ & RQ$^{Th}$ & OSPA$^{Th}$ &PQ$^{St}$&SQ$^{St}$  & RQ$^{St}$ & OSPA$^{St}$\\
%         \hline
% kMaX-DeepLab \cite{yu2022k} & 32.52&77.78&41.38 & [OSPA] &27.96 & 77.23 & 36.00 & [OSPA$^{Th}$] &45.81 & 79.38 & 57.04 & [OSPA$^{St}$]\\
% Mask2Former \cite{cheng2021mask2former} & 33.25&80.53&41.35 & [OSPA] &28.74 & 80.81 & 35.79 & [OSPA$^{Th}$] &46.38 & 79.73 & 57.51 & [OSPA$^{St}$]\\
% Mask DINO \cite{li2023mask} & \textbf{36.57}&\textbf{81.09}&\textbf{44.98} & [OSPA] &\textbf{33.07} & \textbf{81.47} & \textbf{40.56} & [OSPA$^{Th}$] &\textbf{46.74} & \textbf{79.98} & \textbf{57.85} & [OSPA$^{St}$]\\
%         \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Results for panoptic segmentation models (COCO-pretrained) with a ResNet-50 backbone on JRDB panoptic close-world test dataset.}
%     \label{tab:panoptic:closeworld}
% \end{table*}

\begin{table}[!tb]\centering
%\small
    %\begin{adjustbox}{width=0.5\textwidth,center}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l|cc|c|c|}
            \toprule
            
           % \multirow{2}{*}{Method} &
           % \multicolumn{2}{c|}{All (43 classes)} &
            %\multicolumn{2}{c|}{Thing (32 classes)}&
            %\multicolumn{2}{c|}{Stuff (11 classes)}\\
            %\multicolumn{3}{c|}{Mask Size} \\
           % \cmidrule(l{0pt}r{0pt}){2-5}
            Method & PQ  $\uparrow$     & \ospaps $\downarrow$   & \ospaps$^{Th}$   $\downarrow$ &\ospaps$^{St}$ $\downarrow$ \\
            \hline
             ODISE \cite{xu2023open}    &10.57& 0.85&0.90& 0.72\\
            ODISE \cite{xu2023open} (caption)  & 11.07&0.85&0.88&0.78\\
            FC-CLIP \cite{yu2023convolutions} & 8.41&0.87&0.90&0.78\\
            \hline
            FC-CLIP  \cite{yu2023convolutions} $\dotplus$  &\textbf{16.37}&\textbf{0.78} & 0.81&\textbf{0.69}\\
            \bottomrule
        \end{tabular}}
%}\end{adjustbox}
    \caption{Results for current sota open vocabulary panoptic segmentation models on JRDB-Panotrack openworld test set. $\dotplus$ means we trained this model with only JRDB-Panotrack close-world training set.}
    \label{tab:panoptic:openworld}
\end{table}

==> sec/tables/panoptic_open_world_71_old.tex <==

%%% results update 

\begin{table*}[!tb]\centering
% \vspace{-.4cm}
    \centering
    %     \footnotesize
    %         \renewcommand{\arraystretch}{1.6}
    % \resizebox{\columnwidth}{!}{%
    % \resizebox{\textwidth}{!}{%
    \begin{adjustbox}{width=1.0\textwidth,center}
    % \begin{tabular}{l|c|cccccc}
    \begin{tabular}{l|ccc|ccc|ccc|}
    \toprule
    \multirow{2}{*}{Method} & 
    \multicolumn{3}{c|}{All ($71$ classes)}&
    \multicolumn{3}{c|}{Thing ($60$ classes)}&
    \multicolumn{3}{c|}{Stuff ($11$ classes)}\\
    \cmidrule(l{0pt}r{0pt}){2-10}
     &PQ &SQ  & RQ &PQ$^{Th}$ &SQ$^{Th}$ & RQ$^{Th}$ &PQ$^{St}$&SQ$^{St}$  & RQ$^{St}$\\
        \hline     
	

ODISE \cite{xu2023open} &10.57 &56.61&13.17 &7.03 &53.27  &8.72 &29.87 & 74.84 &37.41\\
ODISE \cite{xu2023open} (caption)  & 11.07&61.57&  13.63 & 8.41 & 59.36& 10.26 &25.55& 73.60& 31.98 \\
FC-CLIP \cite{yu2023convolutions} & 10.08&50.76&12.57 &7.11 & 48.32 & 8.82 &26.36 & 64.09 & 33.05\\
FC-CLIP  \cite{yu2023convolutions} $\dotplus$ & \textbf{16.37}&\textbf{62.95}&\textbf{20.15} &\textbf{12.78} & \textbf{59.85} & \textbf{15.71} &\textbf{35.94} & \textbf{79.86} & \textbf{44.38}\\
%FreeSeg (no pretrained model)   & && & & & &&  & \\
        %Mask2Former & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
        %Mask DINO & $52.3$&$58.3$&$43.2$ \\%&$59.5$\\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \centering
    % \vspace{0.2cm}
    \caption{Results for current sota open vocabulary panoptic segmentation models on JRDB test dataset.
    % $\dag$ indicates the box AP is generated from mask prediction.
    % $^*$ indicates it is the test-dev result.
    % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
    % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
    }
    
    \label{tab:panoptic_thing_stuff}
    \vspace{-.4cm}
\end{table*}
